Gradient Estimators for Implicit Models

Implicit models, which allow for the generation of samples but not for point-wise evaluation of probabilities, are omnipresent in real-world problems tackled by machine learning and a hot topic of current research. Some examples include data simulators that are widely used in engineering and scientific research, generative adversarial networks (GANs) for image synthesis, and hot-off-the-press approximate inference techniques relying on implicit distributions. The majority of existing approaches to learning implicit models rely on approximating the intractable distribution or optimisation objective for gradient-based optimisation, which is liable to produce inaccurate updates and thus poor models. This paper alleviates the need for such approximations by proposing the Stein gradient estimator, which directly estimates the score function of the implicitly defined distribution. The efficacy of the proposed estimator is empirically demonstrated by examples that include meta-learning for approximate inference, and entropy regularised GANs that provide improved sample diversity.

==> approximations.tex <==
\section{Gradient approximation with the Stein gradient estimator}
\label{sec:gradient_approximation}

We propose the \emph{Stein gradient estimator} as a novel generalisation of the score matching gradient estimator. Before presenting it we first set-up the notation. Column vectors and matrices are boldfaced. The random variable under consideration is $\x \in \mathcal{X}$ with $\mathcal{X} = \mathbb{R}^{d \times 1}$ if not specifically mentioned. To avoid misleading notation we use the distribution $q(\x)$ to derive the gradient approximations for general cases. As Monte Carlo methods are heavily used for implicit models, in the rest of the paper we mainly consider approximating the gradient $\g(\x^k) :=\nabla_{\x^k} \log q(\x^k)$ for $\x^k \sim q(\x), k = 1, ..., K$. We use $x^i_j$ to denote the $j$th element of the $i$th sample $\x^i$. We also denote the matrix form of the collected gradients as
$\Grad := \left( \nabla_{\x^1} \log q(\x^1), \cdots, \nabla_{\x^K} \log q(\x^K) \right)^{\text{T}} \in \mathbb{R}^{K \times d}$, and its approximation $\hat{\Grad} := \left( \hat{g}(\x^1), \cdots, \hat{g}(\x^K) \right)^{\text{T}}$ with $\hat{g}(\x^k) = \nabla_{\x^k} \log \hat{q}(\x^k)$ for some $\hat{q}(\x)$.

\subsection{KDE gradient estimator: plug-in estimator with kernel density estimation}
A naive approach for gradient approximation would first estimate the intractable density $\hat{q}(\x) \approx q(\x)$ (up to a constant), then approximate the exact gradient by $\nabla_{\x} \log \hat{q}(\x) \approx \nabla_{\x} \log q(\x)$. One may favour complex density approximation schemes for better accuracy, but here we focus on ``quick and dirty'' approximations as the gradient approximation is repeatedly required for the optimisation procedure. Specifically we consider kernel density estimation (KDE) with the reproducing kernel $\mathcal{K}(\x, \cdot)$ of an RKHS $\mathcal{H}$ \citep{berlinet:rkhs2011}, i.e.~
$\hat{q}(\x) = \frac{1}{K} \sum_{k=1}^K \mathcal{K}(\x, \x^k) \times C.$
Simple derivations \citep{singh:kernel_gradient1977} reveal the \emph{KDE gradient estimator} as
\begin{equation}
\hat{\Grad}^{\text{KDE}}_{ij} = \sum_{k=1}^K \nabla_{x^i_j} \mathcal{K}(\x^i, \x^k) / \sum_{k=1}^K \mathcal{K}(\x^i, \x^k).
\label{eq:kde_estimator}
\end{equation}

\subsection{Score matching gradient estimator: minimising MSE}
\label{sec:score_matching}
The KDE estimator performs indirect approximation of the gradient via density estimation, which can be inaccurate. An alternative approach directly approximates the gradient $\nabla_{\x} \log q(\x)$ by minimising the expected $l_2$ error w.r.t.~the approximation $\hat{\g}(\x) = \left(\hat{g}_1(\x), \cdots, \hat{g}_d(\x) \right)^{\text{T}}$:
\begin{equation}
\mathcal{F}(\hat{\g}) := \mathbb{E}_{q} \left[ || \hat{\g}(\x) - \nabla_{\x} \log q(\x) ||_2^2 \right].
\label{eq:fisher_divergence}
\end{equation}
It has been shown in \cite{hyvarinen:score2005} that this objective can be reformulated as
\begin{equation}
\mathcal{F}(\hat{\g}) = \mathbb{E}_{q} \left[ || \hat{\g}(\x) ||_2^2 + 2 \langle \nabla, \hat{\g}(\x) \rangle \right] + C, \quad \langle \nabla, \hat{\g}(\x) \rangle = \sum_{j=1}^d \nabla_{x_j} \hat{g}_j(\x).
\label{eq:score_matching_objective}
i\end{equation}
The key insight here is the usage of integration by parts: after expanding the $l_2$ loss objective, the cross term can be rewritten as
$\mathbb{E}_q \left[ \hat{\g}(\x)^{\text{T}} \nabla_{\x} \log q(\x) \right] = -\mathbb{E}_q \left[ \langle \nabla, \hat{\g}(\x) \rangle \right],$
if assuming the \emph{boundary condition}: $q(\x)\hat{\g}(\x) |_{\partial \mathcal{X}} = \bm{0}$, or $\lim_{\x \rightarrow \bm{\infty}} q(\x)\hat{\g}(\x) = 0$ if $\mathcal{X} = \mathbb{R}^d$. This condition holds for many distributions, e.g.~those with Gaussian-like tails.
%
The optimum of (\ref{eq:score_matching_objective}) is referred as the \emph{score matching gradient estimator}. \cite{sasaki:gradient2014} and \cite{strathmann:kmc2015} derived a parametric solution by first approximating the log density up to a constant with the RBF kernel $\mathcal{K}(\x, \x') := \exp \left[-\frac{1}{2\sigma^2} ||\x - \x' ||_2^2  \right]$, i.e.
$
\log \hat{q}(\x) := \sum_{k=1}^K a_k \mathcal{K}(\x, \x^k) + C$,
then minimising (\ref{eq:score_matching_objective}) to obtain the coefficients $\hat{a}^{\text{score}}_k$ and constructing the gradient estimator as
\begin{equation}
\hat{\Grad}^{\text{score}}_{i\cdot} = \sum_{k=1}^{K} \hat{a}^{\text{score}}_k \nabla_{\x^i} \mathcal{K}(\x^i, \x^k).
\label{eq:grad_parametric_estimator}
\end{equation}
%
A slightly different approach \cite{sasaki:gradient2015} proposes an estimator for $\nabla_{\x} q(\x)$, by minimising the $l_2$ error $\int (\hat{g}_j(\x) - \nabla_{x_j} q(\x))^2 d\x$ and removing explicit calculations of $\nabla_{\x} q(\x)$ in an analogous way as to derive (\ref{eq:score_matching_objective}). 

\subsection{Stein gradient estimator: inverting Stein's identity}
Recall the derivation of the score matching objective (\ref{eq:score_matching_objective}) that uses integration by parts and the boundary condition. Stein's identity \citep{stein:stein_method1972} can also be derived using the same idea . Can we directly exploit Stein's identity to obtain an estimator of the gradients? In this section we investigate the multivariate version of Stein's identity \citep{stein:stein_method_multi1981} to derive a new gradient estimator that we call the \emph{Stein gradient estimator}. 
%
Let $\h: \mathbb{R}^{d \times 1} \rightarrow \mathbb{R}^{d' \times 1}$ be a differentiable multivariate test function satisfying the boundary condition, which maps $\x$ to a column vector $\h(\x) = [h_1(\x), h_2(\x), ..., h_{d'}(\x)]^{\text{T}}$. Now we introduce the multivariate Stein's identity \citep{stein:stein_method_multi1981}
\begin{equation}
\mathbb{E}_{q}[\h(\x) \nabla_{\x} \log q(\x)^{\text{T}} + \nabla_{\x} \h(\x) ] = \bm{0}, 
\label{eq:stein_identity_multi}
\end{equation}
in which the gradient matrix term
$
\nabla_{\x} \h(\x) = \left( \nabla_{\x} h_1(\x), \cdots, \nabla_{\x} h_{d'}(\x) \right)^{\text{T}} \in \mathbb{R}^{d' \times d}.
$
We further approximate the above with Monte Carlo (MC):
\begin{equation}
\frac{1}{K} \sum_{k=1}^K -\h(\x^k) \nabla_{\x^k} \log q(\x^k)^{\text{T}} + \text{err} = \frac{1}{K} \sum_{k=1}^K \nabla_{\x^k} \h(\x^k), \quad \x^k \sim q(\x^k),
\label{eq:stein_multi_mc}
\end{equation}
with $\text{err} \in \mathbb{R}^{d' \times d}$ the random error due to MC approximation, which has mean $\bm{0}$ and vanishes as $K \rightarrow +\infty$. Now by temporarily denoting
$
\Hmatrix = \left( \h(\x^1), \cdots , \h(\x^K) \right) \in \mathbb{R}^{d' \times K}, \quad
\hgrad = \frac{1}{K} \sum_{k=1}^K \nabla_{\x^k} \h(\x^k) \in \mathbb{R}^{d' \times d},
$
equation (\ref{eq:stein_multi_mc}) can be rewritten as
$-\frac{1}{K} \Hmatrix \Grad + \text{err} = \hgrad.$
Thus we consider a ridge regression method (i.e. adding an $l_2$ regulariser) to estimate $\Grad$:
\begin{equation}
\hat{\Grad}_V^{\text{Stein}} := \argmin_{\hat{\Grad} \in \mathbb{R}^{K \times d} } || \hgrad + \frac{1}{K} \Hmatrix \hat{\Grad} ||_{F}^2 + \frac{\eta}{2 K^2} || \hat{\Grad} ||_{F}^2,
\label{eq:stein_objective}
\end{equation}
with $|| \cdot ||_{F}$ the Frobenius norm of a matrix and $\eta \geq 0$. Simple calculation shows that
\begin{equation}
\hat{\Grad}_V^{\text{Stein}} = -( \K + \eta \bm{I} )^{-1} \langle \nabla, \K \rangle,
\label{eq:stein_estimator}
\end{equation}
where $\K := \Hmatrix^{\text{T}} \Hmatrix, \quad \K_{ij} = \mathcal{K}(\x^i, \x^j) := \h(\x^i)^{\text{T}} \h(\x^j),$
$\langle \nabla, \K \rangle := K \Hmatrix^{\text{T}} \hgrad, \quad \langle \nabla, \K \rangle_{ij} = \sum_{k=1}^{K} \nabla_{x^k_j} \mathcal{K}(\x^i, \x^k).$
%
One can show that the RBF kernel satisfies Stein's identity \citep{liu:ksd2016}. In this case $\h(\x) = \mathcal{K}(\x, \cdot), d' = +\infty$ and by the reproducing kernel property,
$\h(\x)^{\text{T}} \h(\x') = \langle \mathcal{K}(\x, \cdot), \mathcal{K}(\x', \cdot) \rangle_{\mathcal{H}} = \mathcal{K}(\x, \x') .$

Interestingly for translation invariant kernels $\mathcal{K}(\x, \x') = \mathcal{K}(\x - \x')$ the KDE gradient estimator (\ref{eq:kde_estimator}) can be rewritten as $\hat{\Grad}^{\text{KDE}} = -\text{diag}\left( \K \bm{1} \right)^{-1} \langle \nabla, \K \rangle.$
Inspecting and comparing it with the Stein gradient estimator (\ref{eq:stein_estimator}), one might notice that the Stein method uses the full kernel matrix as the pre-conditioner, while the KDE method computes an averaged ``kernel similarity'' for the denominator. We conjecture that this difference is key to the superior performance of the Stein gradient estimator when compared to the KDE gradient estimator (see later experiments). The KDE method only collects the similarity information between $\x^k$ and other samples $\x^j$ to form an estimate of $\nabla_{\x^k} \log q(\x^k)$, whereas for the Stein gradient estimator, the kernel similarity between $\x^i$ and $\x^j$ for all $i, j \neq k$ are also incorporated. Thus it is reasonable to conjecture that the Stein method can be more sample efficient, which also implies higher accuracy when the same number of samples are collected.

\subsection{Stein gradient estimator minimises the kernelised Stein discrepancy}
So far we have presented the Stein gradient estimator and compared it to the KDE estimator. In this section we derive the Stein gradient estimator again but from a divergence/discrepancy minimisation perspective. 
%
Stein's method also provides a tool for checking if two distributions $q(\x)$ and $\hat{q}(\x)$ are identical. If the test function set $\mathcal{H}$ is sufficiently rich, then one can define a Stein discrepancy measure by
\begin{equation}
\mathcal{S}(q, \hat{q}) := \sup_{\h \in \mathcal{H}} \mathbb{E}_{q} \left[ \nabla_{\x} \log \hat{q}(\x)^{\text{T}} \h(\x) + \langle \nabla, \h \rangle \right],
\label{eq:stein_discrepancy}
\end{equation}
see \citep{gorham:stein_method2015} for an example derivation. When $\mathcal{H}$ is defined as a unit ball in an RKHS induced by a kernel $\mathcal{K}(\x, \cdot)$, \cite{liu:ksd2016} and \cite{chwialkowski:ksd2016} showed that the supremum in (\ref{eq:stein_discrepancy}) can be analytically obtained as (with $\mathcal{K}_{\x \x'}$ shorthand for $\mathcal{K}(\x, \x')$): 
\begin{equation}
\mathcal{S}^2(q, \hat{q}) = \mathbb{E}_{\x, \x' \sim q} \left[ (\hat{\g}(\x) - \g(\x) )^{\text{T}} \mathcal{K}_{\x \x'} (\hat{\g}(\x') - \g(\x') ) \right],
\end{equation}
which is also named the \emph{kernelised Stein discrepancy} (KSD). \cite{chwialkowski:ksd2016} showed that for $C_0$-universal kernels satisfying the boundary condition, KSD is indeed a discrepancy measure: $\mathcal{S}^2(q, \hat{q}) = 0 \Leftrightarrow q = \hat{q}$.  \cite{gorham:ksd2017} further characterised the power of KSD on detecting non-convergence cases. Furthermore, if the kernel is twice differentiable, then using the same technique as to derive (\ref{eq:score_matching_objective}) one can compute KSD by 
\begin{equation*}
\mathcal{S}^2(q, \hat{q}) = \mathbb{E}_{\x, \x' \sim q} \left[ \hat{\g}(\x)^{\text{T}} \mathcal{K}_{\x \x'} \hat{\g}(\x') + \hat{\g}(\x)^{\text{T}} \nabla_{\x'} \mathcal{K}_{\x \x'} + \nabla_{\x} \mathcal{K}_{\x \x'}^{\text{T}} \hat{\g}(\x') + \text{Tr}(\nabla_{\x, \x'} \mathcal{K}_{\x \x'} )\right].
\end{equation*}
In practice KSD is estimated with samples $\{ \x^k \}_{k=1}^K \sim q$, and simple derivations show that the V-statistic of KSD can be reformulated as $\mathcal{S}_{V}^2(q, \hat{q}) = \frac{1}{K^2} \text{Tr} (\hat{\Grad}^{\text{T}} \K \hat{\Grad} + 2 \hat{\Grad}^{\text{T}} \langle \nabla, \K \rangle) + C$.
%
Thus the $l_2$ error in (\ref{eq:stein_objective}) is equivalent to the V-statistic of KSD if $\h(\x) = \mathcal{K}(\x, \cdot)$, and we have the following:
\begin{theorem}
$\hat{\Grad}_V^{\text{\emph{Stein}}}$ is the solution of the following KSD V-statistic minimisation problem
\begin{equation}
\hat{\Grad}_V^{\text{\emph{Stein}}} = \argmin_{\hat{\Grad} \in \mathbb{R}^{K \times d}} \mathcal{S}_{V}^2(q, \hat{q}) + \frac{\eta}{2 K^2} ||\hat{\Grad}||_F^2 .
\end{equation}
\label{thm:stein_ksd}
\vspace{-0.2in}
\end{theorem}
%
One can also minimise the U-statistic of KSD to obtain gradient approximations, in which we provide a derivation of corresponding optimal solutions in the appendix. In experiments we use V-statistic solutions and leave comparisons between these methods to future work.

The score matching objective (\ref{eq:fisher_divergence}) is also called \emph{Fisher divergence} \citep{johnson:itbook2004} which is a special case of KSD by selecting $\mathcal{K}(\x, \x') = \delta_{\x = \x'}$. Thus the Stein gradient estimator can be viewed as a generalisation of the score matching estimator. The comparison between the two estimators is more complicated. Certainly by the Cauchy-Schwarz inequality the Fisher divergence is stronger than KSD in terms of detecting convergence \citep{liu:ksd2016}. However it is difficult to perform direct gradient estimation by minimising the Fisher divergence as it involves computing second-order gradient terms. Therefore one needs to propose a \emph{parametric} approximation (e.g.~in the form of (\ref{eq:grad_parametric_estimator})) to $\Grad$ and then optimise the associated parameters accordingly, which can remove the advantage of using a stronger divergence potentially.
%
Conversely, the proposed Stein gradient estimator (\ref{eq:stein_estimator}) is \emph{non-parametric} in that it directly optimises over functions evaluated at locations $\{ \x_k \}_{k=1}^K$. 
%
This brings in two key advantages over the score matching gradient estimator: (i) it removes the \emph{approximation error} due to the use of restricted family of parametric approximations and thus can be potentially more accurate; (ii) it has a much simpler and \emph{ubiquitous} form that applies to \emph{any kernel satisfying the boundary condition}, whereas the score matching estimator requires tedious derivations for different kernels repeatedly (see appendix). In terms of computation speed, since in most of the cases the computation of the score matching gradient estimator also involves kernel matrix inversions, both estimators are of the same order of complexity, which is $\mathcal{O}(K^3 + K^2 d)$ (kernel matrix computation plus inversion). Low-rank approximations such as the Nystr\"om method \citep{smola:sparse2000, williams:kernel2001} can enable speed-up, but this is not investigated in the paper.



\subsection{Adding predictive power}
Though providing potentially more accurate approximations, the non-parametric estimator (\ref{eq:stein_estimator}) has no predictive power as described so far. Crucially, many tasks in machine learning require predicting gradient functions at samples sampled from distributions other than $q$, for example, in MLE $q(\x)$ corresponds to the model distribution which is learned using samples from the data distribution instead. To address this issue, hereby we derive two \emph{predictive} estimators, one generalised from the non-parametric estimator and the other minimises KSD using parametric approximations.

\paragraph{Predictions using the non-parametric estimator.}

Let us consider an unseen datum $\y$. If $\y$ is sampled from $q$, then one can also apply the non-parametric estimator (\ref{eq:stein_estimator}) for gradient approximation, given the observed data $\X = \{\x^1, ..., \x^K \} \sim q$. Concretely, if writing $\hat{\g}(\y) \approx \nabla_{\y} \log q(\y) \in \mathbb{R}^{d \times 1}$ then the non-parametric Stein gradient estimator computed on $\X \cup \{\y\}$ is
\begin{equation*}
\begin{bmatrix}
\hat{\g}(\y)^{\text{T}} \\
\hat{\Grad}
\end{bmatrix}
= -( \K^* + \eta \bm{I} )^{-1} 
\begin{bmatrix}
\nabla_{\y} \mathcal{K}(\y, \y) + \sum_{k=1}^{K} \nabla_{\x^k} \mathcal{K}(\y, \x^k) \\
\langle \nabla, \K \rangle + \nabla_{\y} \mathcal{K}(\cdot, \y)
\end{bmatrix}
, \quad 
\K^* = \begin{bmatrix}
    \K_{\y \y}       & \K_{\y\X} \\
    \K_{\X \y}       & \K
\end{bmatrix},
\end{equation*}
with $\nabla_{\y} \mathcal{K}(\cdot, \y)$ denoting a $K \times d$ matrix with rows $\nabla_{\y} \mathcal{K}(\x^k, \y)$, and $\nabla_{\y} \mathcal{K}(\y, \y)$ only differentiates through the second argument. Then we demonstrate in the appendix that, by simple matrix calculations and assuming a translation invariant kernel, we have (with column vector $\bm{1} \in \mathbb{R}^{K \times 1}$):
\begin{equation}
\begin{aligned}
\nabla_{\y} \log q(\y)^{\text{T}} \approx& -\left(\K_{\y\y} + \eta - \K_{\y\X} (\K + \eta \mathbf{I})^{-1} \K_{\X\y} \right)^{-1} \\&\left( \K_{\y\X} \hat{\Grad}_{V}^{\text{Stein}} - \left( \K_{\y\X} (\K + \eta \mathbf{I})^{-1} + \bm{1}^{\text{T}} \right) \nabla_{\y} \mathcal{K}(\cdot, \y) \right).
\end{aligned}
\label{eq:stein_estimator_predict_simplified}
\end{equation}
%
In practice one would store the computed gradient $\hat{\Grad}_{V}^{\text{Stein}}$, the kernel matrix inverse $(\K + \eta \mathbf{I})^{-1}$ and $\eta$ as the ``parameters'' of the predictive estimator.
%
For a new observation $\y \sim p$ in general, one can ``pretend'' $\y$ is a sample from $q$ and apply the above estimator as well. The approximation quality depends on the similarity between $q$ and $p$, and we conjecture here that this similarity measure, if can be described, is closely related to the KSD.
 
\paragraph{Fitting a parametric estimator using KSD.}
The non-parametric predictive estimator could be computationally demanding. Setting aside the cost of fitting the ``parameters'', in prediction the time complexity for the non-parametric estimator is $\mathcal{O}(K^2 + Kd)$. Also storing the ``parameters'' needs $\mathcal{O}(Kd)$ memory for $\hat{\Grad}_{V}^{\text{Stein}}$. These makes the non-parametric estimator undesirable for high-dimensional data, since in order to obtain accurate predictions it often requires $K$ scaling (more than linearly) with $d$ as well. To address this, one can also minimise the KSD using parametric approximations, in a similar way as to derive the score matching estimator in Section \ref{sec:score_matching}. 
%
More precisely, we define a parametric approximation in a similar fashion as (\ref{eq:grad_parametric_estimator}), and in the appendix we show that if the RBF kernel is used for both the KSD and the parametric approximation, then the linear coefficients $\bm{a} = (a_1, ..., a_K)^{\text{T}}$ can be calculated analytically: $\hat{\bm{a}}_{V}^{\text{Stein}} = (\bm{\Lambda} + \eta \mathbf{I})^{-1} \bm{b}$, with
\begin{equation}
\begin{aligned}
\bm{\Lambda} =& \mathbb{X} \odot (\K \K \K) + \K (\K \odot \mathbb{X}) \K - ((\K\K) \odot \mathbb{X}) \K - \K ((\K\K) \odot \mathbb{X}), \\
\bm{b} =& ( \K \text{diag}(\mathbb{X}) \K + (\K \K) \odot \mathbb{X} - \K (\K \odot \mathbb{X}) - (\K \odot \mathbb{X}) \K ) \bm{1},
\end{aligned}
\end{equation}
%
Then for an unseen observation $\y \sim p$ the gradient approximation returns $\nabla_{\y} \log q(\y) \approx (\hat{\bm{a}}^{\text{Stein}}_{V})^{\text{T}} \nabla_{\y} \mathcal{K}(\cdot, \y)$. In this case one only maintains the linear coefficients $\hat{\bm{a}}^{\text{Stein}}_{V}$ and compute a linear combination in prediction, which takes $\mathcal{O}(K)$ memory and $\mathcal{O}(Kd)$ time and therefore it is computationally cheaper than the non-parametric prediction model (\ref{eq:stein_estimator_predict}).



